Using Transfer Learning for Code-Related Tasks

Deep learning (DL) techniques have been used to support several code-related tasks such as code summarization and bug-fixing. In particular, pre-trained transformer models are on the rise, also thanks to the excellent results they achieved in Natural Language Processing (NLP) tasks. The basic idea behind these models is to first pre-train them on a generic dataset using a self-supervised task (e.g, filling masked words in sentences). Then, these models are fine-tuned to support specific tasks of interest (e.g, language translation). A single model can be fine-tuned to support multiple tasks, possibly exploiting the benefits of transfer learning. This means that knowledge acquired to solve a specific task (e.g, language translation) can be useful to boost performance on another task (e.g, sentiment classification). While the benefits of transfer learning have been widely studied in NLP, limited empirical evidence is available when it comes to code-related tasks. In this paper, we assess the performance of the Text-To-Text Transfer Transformer (T5) model in supporting four different code-related tasks: (i) automatic bug-fixing, (ii) injection of code mutants, (iii) generation of assert statements, and (iv) code summarization. We pay particular attention in studying the role played by pre-training and multi-task fine-tuning on the model's performance. We show that (i) the T5 can achieve better performance as compared to state-of-the-art baselines; and (ii) while pre-training helps the model, not all tasks benefit from a multi-task fine-tuning.

==> datasets.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Data Analysis} \label{sec:dataAnalysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section describes the analysis process we performed on our datasets in order to \GABRIELE{@David, Nathan, continue here.} 

The quality of a dataset can dramatically impact the conclusions that are able to be drawn from it. This is because there may be issues related to bias or statistical significance that makes the dataset not suitable for representing the real world. To assess the quality of our datasets we conducted various analsyses around sampling bias and data snooping as recommended in Watson et. al. \REF.

The first analysis is an exploratory data analysis (EDA), which helps answer questions relating to reliability and quality of our datasets. To accomplish this we \NATHAN{@David please fill this in}

The second analysis assesses the level of data snooping among our datasets' training and test sets and how this impacts our model's results. To accomplish this we calculate the overlap between our datasets' training and test sets by first calculating the pairwise Levenshtein Distance \REF between the two sets. With these distances calculated, we next calculate the confidence intervals with a $95\%$ confidence value for each set of distances and determine the amount of overlap between their intervals. We can then take this overlap amount and correlate it with our model's performance to uncover any patterns.

Specifically, we perform a bootstraping analysis where we sampled $30$ times a total of $100$ examples in the training set and $200$ examples in the test set. These $200$ examples from the test set are composed of $100$ the best and $100$ the worst examples in terms of our models performance on the different evaluation metrics (\eg perfect prediction for the program repair task and BLEU score for the code summarization task). Our population of best and worst examples was $1,000$ for each to allow for a diverse set to be sampled from during our bootstrapping.

From this analysis, we would expect to see the model's performance to be worse for test set examples that have low overlap with training examples due to the model having to extrapolate more. However, we found in two task where on average this is not the case, namely the Code Summarization task and the Mutation task. While the differences are quite small, $~0.05$ and $~0.3$ difference in average edit distance for the Code Summarization and Mutation tasks, respectively, it is a suprising finding that requires further investigation. All other tasks performed as expected with the best performing examples having the highest overlap with the training examples and the differences were more pronounced ranging from $1-3$ differences in average edit distance. Lastly, we performed a confidence interval analysis between the best and worst sets and found no overlap between them, except for the Code Summarization task, which had a confidence interval overlap of $~0.012$. This shows that these are indeed two disjoint sets of best performing and worst performing.

\GABRIELE{@David, Nathan describe here. Also, feel free to change the name of this subsection.}
